SMARTIES: user-friendly codes for fast and accurate calculations of light scattering by spheroids

We provide a detailed user guide for SMARTIES, a suite of Matlab codes for the calculation of the optical properties of oblate and prolate spheroidal particles, with comparable capabilities and ease-of-use as Mie theory for spheres. SMARTIES is a Matlab implementation of an improved T-matrix algorithm for the theoretical modelling of electromagnetic scattering by particles of spheroidal shape. The theory behind the improvements in numerical accuracy and convergence is briefly summarised, with reference to the original publications. Instructions of use, and a detailed description of the code structure, its range of applicability, as well as guidelines for further developments by advanced users are discussed in separate sections of this user guide. The code may be useful to researchers seeking a fast, accurate and reliable tool to simulate the near-field and far-field optical properties of elongated particles, but will also appeal to other developers of light-scattering software seeking a reliable benchmark for non-spherical particles with a challenging aspect ratio and/or refractive index contrast.

==> summaryOblate.tex <==
% latex table generated in R 3.2.2 by xtable 1.7-4 package
% Thu Oct 29 14:32:30 2015
\sisetup{detect-all, tight-spacing=false, exponent-product = \cdot,
round-mode = figures,
round-precision = 1}
\thispagestyle{empty}
\begin{table*}[!htpb]
  \label{tab:oblate}
\centering
\scalebox{0.8}{
\begin{tabular}{lllllllllll}
  \toprule[0.15em]
$x_\text{max}$ & \multicolumn{1}{r}{$h$:}   & 1.1 & 1.3 & 2 & 4 & 7 & 10 & 20 & 50 & 100 \\
  \midrule
0.01 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 6 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 100 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 1000 \\ -- \end{tabular} \\
   \midrule
0.10 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 6 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 100 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 1100 \\ -- \end{tabular} \\
   \midrule
1.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 6 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}9 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 90 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 1000 \\ -- \end{tabular} \\
   \midrule
2.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}9 \\ 7 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 100 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 1100 \\ -- \end{tabular} \\
   \midrule
3.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 7 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 100 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 1000 \\ -- \end{tabular} \\
   \midrule
4.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 8 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 10 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 7 \\ \num{2.4e-03} \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 100 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 1100 \\ -- \end{tabular} \\
   \midrule
5.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 8 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 110 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 200 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 550 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 1100 \\ -- \end{tabular} \\
   \midrule
6.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 45 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 110 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 220 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 550 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 1100 \\ -- \end{tabular} \\
   \midrule
7.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 45 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 110 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 220 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 550 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 1100 \\ -- \end{tabular} \\
   \midrule
8.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 10 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 45 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}29 \\ 240 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}29 \\ 600 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 1100 \\ -- \end{tabular} \\
   \midrule
10.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}29 \\ 50 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 90 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}33 \\ 260 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}33 \\ 650 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}33 \\ 1300 \\ -- \end{tabular} \\
   \midrule
12.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 50 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 90 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}33 \\ 130 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}37 \\ 260 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 800 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 1500 \\ -- \end{tabular} \\
   \midrule
15.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}33 \\ 30 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 60 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}37 \\ 100 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 140 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}43 \\ 280 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}39 \\ 700 \\ \num{1.5e-13} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 1400 \\ -- \end{tabular} \\
   \midrule
20.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}37 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 35 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 70 \\ \num{1.0e-13} \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 200 \\ \num{7.4e-12} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 180 \\ \num{4.9e-12} \end{tabular} & \begin{tabular}{@{}l@{}}43 \\ 300 \\ \num{7.0e-13} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 1100 \\ \num{7.5e-13} \end{tabular} & \begin{tabular}{@{}l@{}}53 \\ 1600 \\ -- \end{tabular} \\
   \midrule
25.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 45 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}49 \\ 45 \\ \num{5.1e-13} \end{tabular} & \begin{tabular}{@{}l@{}}51 \\ 70 \\ \num{5.7e-12} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 130 \\ \num{4.0e-11} \end{tabular} & \begin{tabular}{@{}l@{}}43 \\ 180 \\ \num{3.3e-09} \end{tabular} & \begin{tabular}{@{}l@{}}49 \\ 550 \\ \num{1.1e-08} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 900 \\ \num{6.3e-10} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 2000 \\ \num{1.0e-09} \end{tabular} \\
   \midrule
30.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 35 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}53 \\ 30 \\ \num{3.4e-13} \end{tabular} & \begin{tabular}{@{}l@{}}61 \\ 35 \\ \num{2.4e-11} \end{tabular} & \begin{tabular}{@{}l@{}}57 \\ 90 \\ \num{5.0e-10} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 130 \\ \num{3.4e-07} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 200 \\ \num{1.9e-06} \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 400 \\ \num{1.4e-04} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 1200 \\ \num{7.0e-07} \end{tabular} &  \\
   \midrule
40.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}63 \\ 40 \\ \num{2.5e-12} \end{tabular} & \begin{tabular}{@{}l@{}}69 \\ 50 \\ \num{3.9e-10} \end{tabular} & \begin{tabular}{@{}l@{}}75 \\ 50 \\ \num{2.5e-07} \end{tabular} & \begin{tabular}{@{}l@{}}59 \\ 90 \\ \num{7.8e-05} \end{tabular} &  &  &  &  &  \\
   \midrule
50.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}77 \\ 40 \\ \num{5.4e-12} \end{tabular} & \begin{tabular}{@{}l@{}}93 \\ 45 \\ \num{4.4e-08} \end{tabular} & \begin{tabular}{@{}l@{}}103 \\ 45 \\ \num{1.4e-04} \end{tabular} &  &  &  &  &  &  \\
   \midrule
60.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}95 \\ 80 \\ \num{1.8e-09} \end{tabular} & \begin{tabular}{@{}l@{}}115 \\ 500 \\ \num{3.6e-04} \end{tabular} &  &  &  &  &  &  &  \\
   \midrule
70.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}127 \\ 80 \\ \num{1.0e-07} \end{tabular} &  &  &  &  &  &  &  &  \\
   \midrule
80.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}111 \\ 1200 \\ \num{7.4e-05} \end{tabular} &  &  &  &  &  &  &  &  \\
   \bottomrule[0.15em]
\end{tabular}
}
\caption{Convergence study for an oblate spheroid with $s= 1.311+0i$. For each pair of size parameter $x_\text{max}$ (rows) and aspect ratio $h$ (columns), we list the convergence parameters $N, N_\theta$. The relative error is only displayed if higher than $10^{-13}$.}
\end{table*}


==> summaryProlate.tex <==
% latex table generated in R 3.2.2 by xtable 1.7-4 package
% Thu Oct 29 14:32:30 2015
\sisetup{detect-all, tight-spacing=false, exponent-product = \cdot,
round-mode = figures,
round-precision = 1}
\thispagestyle{empty}
\begin{table*}[!htpb]
  \label{tab:prolate}
\centering
\scalebox{0.8}{
\begin{tabular}{lllllllllll}
  \toprule[0.15em]
$x_\text{max}$ & \multicolumn{1}{r}{$h$:}   & 1.1 & 1.3 & 2 & 4 & 7 & 10 & 20 & 50 & 100 \\
  \midrule
0.01 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 6 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 220 \\ \num{2.2e-13} \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 650 \\ \num{4.8e-13} \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 800 \\ \num{2.9e-12} \end{tabular} \\
   \midrule
0.10 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 6 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}5 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 220 \\ \num{2.2e-13} \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 650 \\ \num{4.8e-13} \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 800 \\ \num{2.9e-12} \end{tabular} \\
   \midrule
1.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}7 \\ 6 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}9 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 220 \\ \num{1.8e-13} \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 650 \\ \num{4.0e-13} \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 800 \\ \num{2.3e-12} \end{tabular} \\
   \midrule
2.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}9 \\ 7 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 260 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 400 \\ \num{5.1e-13} \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 800 \\ \num{1.4e-12} \end{tabular} \\
   \midrule
3.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 7 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}11 \\ 9 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 220 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 800 \\ \num{5.9e-13} \end{tabular} \\
   \midrule
5.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}13 \\ 8 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}15 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 40 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 70 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 220 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 500 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 1000 \\ \num{3.1e-13} \end{tabular} \\
   \midrule
7.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}17 \\ 10 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}19 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 45 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 220 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 650 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 1000 \\ \num{1.5e-13} \end{tabular} \\
   \midrule
10.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}21 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}23 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}25 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 45 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 80 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 120 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 260 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 600 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 1400 \\ -- \end{tabular} \\
   \midrule
15.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}27 \\ 15 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}31 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}33 \\ 30 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 60 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}37 \\ 90 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}37 \\ 140 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}39 \\ 280 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}39 \\ 700 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}39 \\ 1600 \\ -- \end{tabular} \\
   \midrule
20.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}35 \\ 20 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}37 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 30 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}43 \\ 90 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}43 \\ 120 \\ \num{3.1e-13} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 160 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 300 \\ \num{2.4e-13} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 900 \\ \num{4.7e-13} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 1800 \\ \num{8.1e-13} \end{tabular} \\
   \midrule
25.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}41 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}49 \\ 45 \\ \num{2.4e-12} \end{tabular} & \begin{tabular}{@{}l@{}}49 \\ 70 \\ \num{2.6e-12} \end{tabular} & \begin{tabular}{@{}l@{}}43 \\ 120 \\ \num{2.6e-10} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 160 \\ \num{2.4e-10} \end{tabular} & \begin{tabular}{@{}l@{}}49 \\ 350 \\ \num{8.9e-11} \end{tabular} & \begin{tabular}{@{}l@{}}53 \\ 1100 \\ \num{3.4e-12} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 2000 \\ \num{1.7e-11} \end{tabular} \\
   \midrule
30.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 25 \\ -- \end{tabular} & \begin{tabular}{@{}l@{}}53 \\ 30 \\ \num{9.7e-13} \end{tabular} & \begin{tabular}{@{}l@{}}61 \\ 45 \\ \num{4.8e-11} \end{tabular} & \begin{tabular}{@{}l@{}}49 \\ 100 \\ \num{7.0e-10} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 130 \\ \num{1.3e-08} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 200 \\ \num{1.2e-08} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 350 \\ \num{2.5e-07} \end{tabular} & \begin{tabular}{@{}l@{}}45 \\ 1200 \\ \num{2.0e-07} \end{tabular} & \begin{tabular}{@{}l@{}}47 \\ 2000 \\ \num{1.7e-08} \end{tabular} \\
   \midrule
40.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}67 \\ 40 \\ \num{1.6e-12} \end{tabular} & \begin{tabular}{@{}l@{}}73 \\ 40 \\ \num{1.1e-10} \end{tabular} & \begin{tabular}{@{}l@{}}89 \\ 40 \\ \num{4.1e-08} \end{tabular} & \begin{tabular}{@{}l@{}}59 \\ 110 \\ \num{6.7e-07} \end{tabular} &  &  &  &  &  \\
   \midrule
50.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}79 \\ 60 \\ \num{4.5e-11} \end{tabular} & \begin{tabular}{@{}l@{}}95 \\ 45 \\ \num{6.9e-08} \end{tabular} & \begin{tabular}{@{}l@{}}113 \\ 50 \\ \num{7.3e-05} \end{tabular} &  &  &  &  &  &  \\
   \midrule
60.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}97 \\ 45 \\ \num{8.0e-10} \end{tabular} & \begin{tabular}{@{}l@{}}117 \\ 180 \\ \num{1.7e-04} \end{tabular} &  &  &  &  &  &  &  \\
   \midrule
70.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}87 \\ 70 \\ \num{2.6e-07} \end{tabular} &  &  &  &  &  &  &  &  \\
   \midrule
80.00 & \begin{tabular}{@{}l@{}}N \\ $N_\theta$ \\ \emph{error} \end{tabular} & \begin{tabular}{@{}l@{}}109 \\ 120 \\ \num{1.0e-04} \end{tabular} &  &  &  &  &  &  &  &  \\
   \bottomrule[0.15em]
\end{tabular}
}
\caption{Convergence study for a prolate spheroid with $s= 1.311+0i$. For each pair of size parameter $x_\text{max}$ (rows) and aspect ratio $h$ (columns), we list the convergence parameters $N, N_\theta$. The relative error is only displayed if higher than $10^{-13}$.}
\end{table*}

